Reducing the Complexity of Quantified Formulas via Variable Elimination

We present a general simplification of quantified SMT formulas using variable elimination. The simplification is based on an analysis of the ground terms occurring as arguments in function applications. We use this information to generate a system of set constraints, which is then solved to compute a set of sufficient ground terms for each variable. Universally quantified variables with a finite set of sufficient ground terms can be eliminated by instantiating them with the computed ground terms. The resulting SMT formula contains potentially fewer quantifiers and thus is potentially easier to solve. We describe how a satisfying model of the resulting formula can be modified to satisfy the original formula. Our experiments show that in many cases, this simplification considerably improves the solving time, and our evaluations using Z3 and CVC4 indicate that the idea is not specific to a particular solver, but can be applied in general.

==> experiments.tex <==
% !TEX root =  a.a.elghazi_m.taghdiri_smt2013.draft02.tex
\section{Experiment Results}
\label{a:sect:experiments}

\achraf{[Change the number of sufGT:50 with the ones of suGT:comp] done}\\

\achraf{[Modify the text of drop it]}

To evaluate the efficiency of our in \ref{sect:sufGTSets} described variable elimination and their in \ref{sect:optimization} described improvements, the approach have been prototypical implemented and evaluated with the SMT-COMP benchmarks of 2012 using the CVC4 and Z3 as benchmark SMT solvers. 
From all benchmarks of the SMT-COMP/AUFLIA-p 2012, we have chosen all benchmarks with a runtime\footnote{At the SMT-COMP} $\ge 1$ second using Z3, or $\ge 10$ seconds using CVC3 or CVC4. 
For each benchmark in our evaluation set we compare its runtime without and with our simplification using two different configurations for $IQ_{max}$, $20$ and  $\infty$.

Table ?
%\ref{tab:cvc4-results} 
gives the comparison results for CVC4 (version 1.0), and Table ?
%\ref{tab:z3-results} 
the results for Z3 (version 4.1).
The \emph{Time} column denotes the solver runtime measured on an Intel Core2Quad, $2.8$GHz, $8$GB memory. The two results in the second \emph{Time} column denote the results of the two simplification configurations with $BIQ_{max}$ set to $20$ / $50$ respectively. The \emph{Result} column gives the outcome of the run: ``unsat'' if the solver can prove the unsatisfiability of the benchmark, ``sat'' if it can find a model for the benchmark, ``UK'' if the solver returns ``unknown'', and ``--'' if it reaches the time-out (\emph{TO}) of $600$ seconds.

If we count $600$ seconds for each time-out, we get a total time of $53730$ seconds, spent by CVC4 to solve all $131$ benchmarks without simplification. Applying the sufGT simplification, the total time could be reduced to $48959$ seconds with $BIQ_{max} = 20$, a speed up of $1.09$, and to $47803$ with $BIQ_{max} = 50$, a speed up of $1.12$. For Z3, the total time spent to solve all benchmarks was $4132$ seconds, which could be reduced to $3302$ seconds with $BIQ_{max} = 20$, a speedup of $1.25$, and to $3300$ seconds with $BIQ_{max} = 50$, a speedup of also $1.25$. An other important aspect is the time-out statistic. In this respect, CVC3 times out $87$ times without simplification, but only $74$ times using the sugGT simplification for $BIQ_{max} = 20$ and only $76$ times for $BIQ_{max} = 50$. Z3 times out $6$ times without simplification, but only $5$ times using the sufGT simplification for $BIQ_{max} = 20$ and also $5$ times for $BIQ_{max} = 50$.




\begin{table}[htbp]
\label{tab:cvc4-results}
\begin{minipage}{0.60\textwidth}
\centering
\resizebox {1\textwidth }{!}{
\begin{tabular}[c]{c c!{\vrule width 1.5pt}c|c!{\vrule width 1.5pt}c|c|}
\cline{3-6} %\hline
& &\multicolumn{2}{c!{\vrule width 1.5pt}}{\textsc{CVC4V1.0}} & \multicolumn{2}{c|}{\textsc{CVC4V1.0$_{sufGT_{Conf2'}}$}}  \\
\hline                                                                                                                                                                                                                             
\multicolumn{1}{|c|}{\textsc{Category}}	& \textsc{Benchmark} & \textsc{Time} & \textsc{Result}	& \textsc{Time} & \textsc{Result}  \\
\hline                                                                                                                                                                                                                  
%                                                                                                             
% boogie                                                                                                             
%                                                                                                             
\multicolumn{1}{|c|}{boogie}	 	& AssignToNonInvariantField\_AnotherClient.P\_AlsoGood       & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& Assumptions\_Assumptions.Swap\_System.Boolean   	     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& BClient\_Client.P\_MyClass\_notnull   	    	     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& Bag5\_Bag..ctor\_System.Int32.array\_notnull   	     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& Bag8\_Bag..ctor\_System.Int32.array\_notnull   	     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& Bag9\_Bag.Add\_System.Int32   	    	     	     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& Chunker11b\_Chunker..System.String\_notnull\_System.Int32  & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& ExposeVersion\_QClient..ctor-level\_2   	    	     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& LocalExpose\_T.V0   	    	     			     & 291  & unsat   & 21  / 14       & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& ManualRange1\_Tools.Range\_Enumerator..Int32\_System.Int32 & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& PeerFields\_Parent.Assign1   	    	      		     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& PeerFields\_PeerFields.Assign0   	    	     	     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& PeerFields\_PeerFields.Assign1\_PeerFields   	    	     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& QuantifierVisibilityInvariant\_A..ctor   	    	     & TO   & --      & 22  / 3        & unsat / unsat     \\
\hline                                                                                                                                                 
\multicolumn{1}{|c|}{sexpr}	 	& SES.Atom..ctor\_SES.Atom\_notnull\_System.Boolean 	     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 	        	& SES.Atom.Write\_System.IO.TextWriter\_notnull       	     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 	        	& SES.Nary.FA\_System.Cl.G.List\_1..Cn.NNT.SES.Sx\_notnull   & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 	        	& SES.Nary.JunctionFA\_System.Bool..Cn.NNT.SES.Sx\_notnull   & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& SES.PrettySx.SkipWhiteSpace\_System..System.IO.TextWriter  & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 	        	& SES.PrettySx.Write\_SES.Sx..System.IO.TextWriter\_notnull  & TO   & --      & 56  / 56       & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}   		& SES.Sx.get\_True    					     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}   		& SiblingConstructors..ctor\_System.Int32\_System.Boolean    & 70   & unsat   & 100 / 7        & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}   		& Spouse\_Person.B2    					     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}   		& Spouse\_Person.Marry\_CaptureEither\_Person\_notnull       & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}   		& Spouse\_Person.Marry\_Person\_notnull    		     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}   		& Strings\_test3.MyStrings.StringCoolness2\_System.Boolean   & TO   & --      & 147 / TO       & unsat / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}   		& VisibilityBasedInvariants\_Friend..ctor\_Thing\_notnull    & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}   		& VisibilityBasedInvariants\_Thing.P    		     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}   		& VisibilityBasedInvariants\_Thing.Q    		     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}   		& VisibilityBasedInvariants\_Thing.R    		     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}   		& WhereMotivation\_Types.MLoop3    			     & TO   & --      & TO  / TO       & --    / --        \\
\hline                                                                                                                                                 
\multicolumn{1}{|c|}{simplify1/2} 	& javafe.PrintSpec.005		    			     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.PrintSpec.014		    			     & 3    & unsat   & 1   / 2        & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.ast.ArrayRefExpr.001 	    			     & TO   & --      & 1   / TO       & unsat / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.ast.ArrayType.44	    			     & TO   & --      & 0   / 1        & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.ast.CompilationUnit.85	    			     & TO   & --      & 1   / TO       & unsat / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.ast.CompoundName.96    			     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.ast.ConstructorInvocation.003    		     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.ast.ExprVec.005	    			     & 1    & unsat   & 1   / 2        & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.ast.ExprVec.009 	    			     & 2    & unsat   & 9   / 9        & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.ast.ExprVec.018	   			     & 47   & unsat   & 10  / 12       & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.ast.ForStmt.003	    			     & 8    & unsat   & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.ast.FormalParaDeclVec.002			     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.ast.FormalParaDeclVec.016		             & 0    & unsat   & 2   / 2        & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.ast.IdentifierVec.012    			     & 17   & unsat   & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.ast.ImportDeclVec.015	    			     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.ast.InterfaceDecl.207	    			     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.ast.MethodInvocation.003    			     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.ast.MethodInvocation.245    			     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.ast.ModifierPragmaVec.009  			     & 1    & unsat   & 10  / 8        & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.ast.ModifierPragmaVec.252    			     & 12   & unsat   & 17  / 16       & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			&  javafe.ast.PrimitiveType.292   			     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			&  javafe.ast.StandardPrettyPrint.004   		     & 3    & unsat   & 2   / 3        & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.ast.StandardPrettyPrint.005    		     & TO   & --      & 64  / 60       & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.ast.StandardPrettyPrint.014    		     & 2    & unsat   & 3   / 5        & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.ast.StandardPrettyPrint.016    		     & 14   & unsat   & 10  / 13       & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.ast.StmtVec.005		  		     & 2    & unsat   & 0   / 0        & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.ast.TypeDeclVec.001	    			     & TO   & --      & 17  / TO       & unsat / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.ast.TypeModifierPragmaVec.021 			     & 0    & unsat   & 1   / 1        & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.ast.TypeNameVec.018				     & 47   & unsat   & 11  / 12       & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.ast.VarInitVec.002		   		     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.ast.VarInitVec.018		   		     & 42   & unsat   & 10  / 13       & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.ast.VarInitVec.021	    			     & 0    & unsat   & 1   / 1        & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.parser.Lex.009		    			     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.parser.Lex.011		    			     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.parser.Lex.012    				     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.parser.Parse.003		  		     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.parser.Parse.005		   		     & TO   & --      & 192 / TO       & unsat / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.parser.Parse.006		   		     & TO   & --      & 497 / 139      & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.parser.ParseExpr.003		   		     & TO   & --      & 309 / TO       & unsat / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.parser.ParseExpr.006	    			     & TO   & --      & 406 / TO       & unsat / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.parser.ParseExpr.014		   		     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.parser.ParseStmt.004	    			     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{}		 	& javafe.parser.ParseStmt.007	    			     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.parser.ParseStmt.009		   		     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.parser.ParseStmt.010		   		     & TO   & --      & TO  / 13       & --    / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.parser.ParseType.564		   		     & TO   & --      & 275 / 282      & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.parser.ParseUtil.566		   		     & 18   & unsat   & 176 / 172      & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.parser.ParseUtil.567		   		     & 28   & unsat   & 128 / 124      & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.parser.test.TestLex.009	   		     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.parser.test.TestLex.017	   		     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.parser.test.TestLex.025	   		     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.parser.test.TestLex.033	   		     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.reader.SrcReader.614		   		     & 100  & unsat   & 0   / 0        & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.tc.CheckInvariants.003		   		     & 9    & unsat   & 9   / 8        & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.tc.CheckInvariants.637		   		     & 11   & unsat   & 9   / 11       & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.tc.ConstantExpr.002		   		     & 20   & unsat   & 5   / 6        & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.tc.Env.005			   		     & 1    & unsat   & 2   / 3        & unsat / unsat     \\
\cline{2-6}                                                                                                                                            
\multicolumn{1}{|c|}{} 			& javafe.tc.Env.006			   		     & TO   & --      & 403 / TO       & unsat / --        \\
\end{tabular}
} % End of \resizebox
\end{minipage}
\begin{minipage}{0.60\textwidth}
\centering
\resizebox {1\textwidth}{!}{
\begin{tabular}[c]{c c!{\vrule width 1.5pt}c|c!{\vrule width 1.5pt}c|c|}
\multicolumn{1}{|c|}{} 			& javafe.tc.EnvForCU.007		     		     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& javafe.tc.FlowInsensitiveChecks.011	   		     & 2    & unsat   & 2   / 3        & unsat / unsat     \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& javafe.tc.FlowInsensitiveChecks.014   		     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& javafe.tc.FlowInsensitiveChecks.017   		     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& javafe.tc.FlowInsensitiveChecks.018   		     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& javafe.tc.FlowInsensitiveChecks.025   		     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& javafe.tc.FlowInsensitiveChecks.027	   		     & 2    & unsat   & 2   / 3        & unsat / unsat     \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{}		 	& javafe.tc.FlowInsensitiveChecks.687  			     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& javafe.tc.MethodDeclVec.698		   		     & 80   & unsat   & 28  / 65       & unsat / unsat     \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& javafe.tc.OutsideEnv.009		   		     & 28   & unsat   & 70  / 22       & unsat / unsat     \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{}		 	& javafe.tc.PrepTypeDeclaration.001	    		     & TO   & --      & TO  / TO       & unsat / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& javafe.tc.PrepTypeDeclaration.005	   		     & 10   & unsat   & 12  / TO       & unsat / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{}		 	& javafe.tc.PrepTypeDeclaration.010   			     & TO   & --      & TO  / TO       & unsat / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{}		 	& javafe.tc.PrepTypeDeclaration.011    			     & TO   & --      & TO  / TO       & unsat / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{}		 	& javafe.tc.PrepTypeDeclaration.013    			     & TO   & --      & 430 / TO       & unsat / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{}		 	& javafe.tc.PrepTypeDeclaration.014    			     & TO   & --      & EX  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& javafe.tc.PrepTypeDeclaration.017	   		     & 2    & unsat   & 3   / 5        & unsat / unsat     \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{}		 	& javafe.tc.PrepTypeDeclaration.705    			     & TO   & --      & TO  / TO       & unsat / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{}		 	& javafe.tc.PrepTypeDeclaration.709    			     & TO   & --      & TO  / TO       & unsat / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& javafe.tc.SLResolution.001		   		     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& javafe.tc.TypeCheck.011		   		     & 3    & unsat   & 3   / 2        & unsat / unsat     \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& javafe.tc.TypeCheck.012		   		     & 3    & unsat   & 4   / 2        & unsat / unsat     \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& javafe.tc.TypeCheck.015		   		     & 2    & unsat   & 1   / 2        & unsat / unsat     \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{}		 	& javafe.tc.TypeSig.002		    			     & TO   & --      & 14  / TO       & unsat / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{}		 	& javafe.tc.TypeSig.729		    			     & TO   & --      & 3   / 6        & unsat / unsat     \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& javafe.tc.TypeSigVec.009		   		     & TO   & --      & 42  / 59       & unsat / unsat     \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& javafe.tc.TypeSigVec.740		   		     & 10   & unsat   & 9   / TO       & unsat / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{}		 	& javafe.tc.Types.053		    			     & 584  & unsat   & TO  / TO       & unsat / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& javafe.util.LocationManagerCorrelatedReader.800   	     & 5    & unsat   & 137 / 5        & unsat / unsat     \\
\hline                                                                                                                                                  
\multicolumn{1}{|c|}{misc} 		& list1    						     & 0    & unsat   & 0   / 0        & unsat / unsat     \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& list4    						     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& list6    						     & 0    & UK      & 3   / 0        & UK    / UK   \\
\hline                                                                                                                                                  
\multicolumn{1}{|c|}{boogie}		& loopinv0\_LoopInv0.Method0-infer\_eh 			     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{}		 	& loopinv0\_LoopInv0.Method2\_Node\_notnull-infer\_eh	     & TO   & unsat   & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{}		 	& loopinv3\_Foreach.M\_System.Int32.array\_notnull-infer\_eh & 49   & unsat   & 396 / 395      & unsat / unsat     \\
\hline                                                                                                                                                  
\multicolumn{1}{|c|}{misc} 		& set14    						     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& set16    						     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& set19    						     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& set1    					             & 2    & unsat   & 0   / 0        & unsat / unsat     \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& set2    						     & TO   & --      & TO  / TO       & --    / --        \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& set3    						     & 0    & unsat   & 0   / 0        & unsat / unsat     \\
\cline{2-6}                                                                                                                                             
\multicolumn{1}{|c|}{} 			& set9    						     & TO   & --      & TO  / TO       & --    / --        \\
\hline                                                                                                                                                                                            
\end{tabular}
} % End of \resizebox
\end{minipage}
\caption{Experiment results of running CVC4 on Z3/CVCx difficult ($\ge$1/$\ge$10) benchmarks of the SMT-COMP/AUFLIA-p without and with the \emph{sufGT} simplification}
\end{table}




\begin{table}[htbp]
\label{tab:z3-results}
\begin{minipage}{0.60\textwidth}
\centering
\resizebox {1\textwidth }{!}{
\begin{tabular}[c]{c c!{\vrule width 1.5pt}c|c!{\vrule width 1.5pt}c|c|}
\cline{3-6} %\hline
& &\multicolumn{2}{c!{\vrule width 1.5pt}}{\textsc{Z3V4.1}} & \multicolumn{2}{c|}{\textsc{Z3V4.1$_{sufGT_{Conf2'}}$}}  \\
\hline                                                                                                                                                                                                                             
\multicolumn{1}{|c|}{\textsc{Category}}	& \textsc{Benchmark} & \textsc{Time} & \textsc{Result}	& \textsc{Time} & \textsc{Result}  \\
\hline                                                                                                                                                                                                                  
%                                                                                                             
% boogie                                                                                                             
%                                                                                                             
\multicolumn{1}{|c|}{boogie}	 	& AssignToNonInvariantField\_AnotherClient.P\_AlsoGood        & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& Assumptions\_Assumptions.Swap\_System.Boolean   	      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& BClient\_Client.P\_MyClass\_notnull   	    	      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& Bag5\_Bag..ctor\_System.Int32.array\_notnull   	      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& Bag8\_Bag..ctor\_System.Int32.array\_notnull   	      & 0    & unsat   & 1  / 1    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& Bag9\_Bag.Add\_System.Int32   	    	     	      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& Chunker11b\_Chunker..System.String\_notnull\_System.Int32   & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& ExposeVersion\_QClient..ctor-level\_2   	    	      & 1    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& LocalExpose\_T.V0   	    	     			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& ManualRange1\_Tools.Range\_Enumerator..Int32\_System.Int32  & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& PeerFields\_Parent.Assign1   	    	      		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& PeerFields\_PeerFields.Assign0   	    	     	      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& PeerFields\_PeerFields.Assign1\_PeerFields   	    	      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& QuantifierVisibilityInvariant\_A..ctor   	    	      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\hline                                                                                                                                             
\multicolumn{1}{|c|}{sexpr}	 	& SES.Atom..ctor\_SES.Atom\_notnull\_System.Boolean 	      & 264  & unsat   & 9  / 9    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 	        	& SES.Atom.Write\_System.IO.TextWriter\_notnull       	      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 	        	& SES.Nary.FA\_System.Cl.G.List\_1..Cn.NNT.SES.Sx\_notnull    & 8    & unsat   & 4  / 4    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 	        	& SES.Nary.JunctionFA\_System.Bool..Cn.NNT.SES.Sx\_notnull    & 19   & unsat   & 3  / 3    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& SES.PrettySx.SkipWhiteSpace\_System..System.IO.TextWriter   & --   & TO      & 7  / 7    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 	        	& SES.PrettySx.Write\_SES.Sx..System.IO.TextWriter\_notnull   & 37   & unsat   & 2  / 2    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}   		& SES.Sx.get\_True    					      & 6    & unsat   & 3  / 3    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}   		& SiblingConstructors..ctor\_System.Int32\_System.Boolean     & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}   		& Spouse\_Person.B2    					      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}   		& Spouse\_Person.Marry\_CaptureEither\_Person\_notnull        & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}   		& Spouse\_Person.Marry\_Person\_notnull    		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}   		& Strings\_test3.MyStrings.StringCoolness2\_System.Boolean    & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}   		& VisibilityBasedInvariants\_Friend..ctor\_Thing\_notnull     & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}   		& VisibilityBasedInvariants\_Thing.P    		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}   		& VisibilityBasedInvariants\_Thing.Q    		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}   		& VisibilityBasedInvariants\_Thing.R    		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}   		& WhereMotivation\_Types.MLoop3    			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\hline                                                                                                                                             
\multicolumn{1}{|c|}{simplify1/2} 	& javafe.PrintSpec.005		    			      & 0    & unsat   & 0  / 5    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.PrintSpec.014		    			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.ast.ArrayRefExpr.001 	    			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.ast.ArrayType.44	    			      & 0    & unsat   & 0  / 14   & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.ast.CompilationUnit.85	    			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.ast.CompoundName.96    			      & 0    & unsat   & 0  / 1    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.ast.ConstructorInvocation.003    		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.ast.ExprVec.005	    			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.ast.ExprVec.009 	    			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.ast.ExprVec.018	   			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.ast.ForStmt.003	    			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.ast.FormalParaDeclVec.002			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.ast.FormalParaDeclVec.016		              & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.ast.IdentifierVec.012    			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.ast.ImportDeclVec.015	    			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.ast.InterfaceDecl.207	    			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.ast.MethodInvocation.003    			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.ast.MethodInvocation.245    			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.ast.ModifierPragmaVec.009  			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.ast.ModifierPragmaVec.252    			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			&  javafe.ast.PrimitiveType.292   			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			&  javafe.ast.StandardPrettyPrint.004   		      & 0    & unsat   & 0  / 1    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.ast.StandardPrettyPrint.005    		      & 1    & unsat   & 0  / 2    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.ast.StandardPrettyPrint.014    		      & 0    & unsat   & 0  / 1    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.ast.StandardPrettyPrint.016    		      & 0    & unsat   & 0  / 2    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.ast.StmtVec.005		  		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.ast.TypeDeclVec.001	    			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.ast.TypeModifierPragmaVec.021 			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.ast.TypeNameVec.018				      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.ast.VarInitVec.002		   		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.ast.VarInitVec.018		   		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.ast.VarInitVec.021	    			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.parser.Lex.009		    			      & 0    & unsat   & 0  / 3    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.parser.Lex.011		    			      & 0    & unsat   & 1  / 2    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.parser.Lex.012    				      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.parser.Parse.003		  		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.parser.Parse.005		   		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.parser.Parse.006		   		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.parser.ParseExpr.003		   		      & 0    & unsat   & 0  / 1    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.parser.ParseExpr.006	    			      & 0    & unsat   & 0  / 1    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.parser.ParseExpr.014		   		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.parser.ParseStmt.004	    			      & 0    & unsat   & 0  / 1    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{}		 	& javafe.parser.ParseStmt.007	    			      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.parser.ParseStmt.009		   		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.parser.ParseStmt.010		   		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.parser.ParseType.564		   		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.parser.ParseUtil.566		   		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.parser.ParseUtil.567		   		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.parser.test.TestLex.009	   		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.parser.test.TestLex.017	   		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.parser.test.TestLex.025	   		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.parser.test.TestLex.033	   		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.reader.SrcReader.614		   		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.tc.CheckInvariants.003		   		      & 0    & unsat   & 0  / 1    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.tc.CheckInvariants.637		   		      & 1    & unsat   & 1  / 3    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.tc.ConstantExpr.002		   		      & 0    & unsat   & 0  / 1    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.tc.Env.005			   		      & 0    & unsat   & 0  / 0    & unsat / unsat  \\
\cline{2-6}                                                                                                                                        
\multicolumn{1}{|c|}{} 			& javafe.tc.Env.006			   		      & 0    & unsat   & 0  / 1    & unsat / unsat  \\
\end{tabular}
} % End of \resizebox
\end{minipage}
\begin{minipage}{0.60\textwidth}
\centering
\resizebox {1\textwidth}{!}{
\begin{tabular}[c]{c c!{\vrule width 1.5pt}c|c!{\vrule width 1.5pt}c|c|}
\multicolumn{1}{|c|}{} 			& javafe.tc.EnvForCU.007		     		      & 0    & unsat   & 0  / 0    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& javafe.tc.FlowInsensitiveChecks.011	   		      & 0    & unsat   & 0  / 0    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& javafe.tc.FlowInsensitiveChecks.014   		      & 0    & unsat   & 0  / 1    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& javafe.tc.FlowInsensitiveChecks.017   		      & 0    & unsat   & 0  / 0    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& javafe.tc.FlowInsensitiveChecks.018   		      & 0    & unsat   & 0  / 0    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& javafe.tc.FlowInsensitiveChecks.025   		      & 0    & unsat   & 0  / 0    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& javafe.tc.FlowInsensitiveChecks.027	   		      & 0    & unsat   & 0  / 0    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{}		 	& javafe.tc.FlowInsensitiveChecks.687  			      & 0    & unsat   & 0  / 1    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& javafe.tc.MethodDeclVec.698		   		      & 0    & unsat   & 0  / 0    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& javafe.tc.OutsideEnv.009		   		      & 0    & unsat   & 0  / 0    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{}		 	& javafe.tc.PrepTypeDeclaration.001	    		      & 5    & unsat   & 0  / 193  & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& javafe.tc.PrepTypeDeclaration.005	   		      & 0    & unsat   & 0  / 0    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{}		 	& javafe.tc.PrepTypeDeclaration.010   			      & 0    & unsat   & 0  / 1    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{}		 	& javafe.tc.PrepTypeDeclaration.011    			      & 0    & unsat   & 0  / 0    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{}		 	& javafe.tc.PrepTypeDeclaration.013    			      & 0    & unsat   & 0  / 0    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{}		 	& javafe.tc.PrepTypeDeclaration.014    			      & 0    & unsat   & 0  / 1    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& javafe.tc.PrepTypeDeclaration.017	   		      & 0    & unsat   & 0  / 1    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{}		 	& javafe.tc.PrepTypeDeclaration.705    			      & 2    & unsat   & 0  / 187  & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{}		 	& javafe.tc.PrepTypeDeclaration.709    			      & 0    & unsat   & 0  / 1    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& javafe.tc.SLResolution.001		   		      & 0    & unsat   & 0  / 71   & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& javafe.tc.TypeCheck.011		   		      & 0    & unsat   & 0  / 0    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& javafe.tc.TypeCheck.012		   		      & 0    & unsat   & 0  / 0    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& javafe.tc.TypeCheck.015		   		      & 0    & unsat   & 0  / 0    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{}		 	& javafe.tc.TypeSig.002		    			      & 0    & unsat   & 0  / 69   & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{}		 	& javafe.tc.TypeSig.729		    			      & 0    & unsat   & 0  / 1    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& javafe.tc.TypeSigVec.009		   		      & 0    & unsat   & 0  / 1    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& javafe.tc.TypeSigVec.740		   		      & 0    & unsat   & 0  / 0    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{}		 	& javafe.tc.Types.053		    			      & 0    & unsat   & 0  / 109  & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& javafe.util.LocationManagerCorrelatedReader.800   	      & 0    & unsat   & 0  / 0    & unsat / unsat   \\
\hline                                                                                                                                               
\multicolumn{1}{|c|}{misc} 		& list1    						      & 0    & unsat   & 0  / 0    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& list4    						      & --   & TO      & TO / TO   & --    / --      \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& list6    						      & --   & TO      & TO / TO   & --    / --      \\
\hline                                                                                                                                               
\multicolumn{1}{|c|}{boogie}		& loopinv0\_LoopInv0.Method0-infer\_eh 			      & 0    & unsat   & 0  / 0    & unsat / unsat   \\ 
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{}		 	& loopinv0\_LoopInv0.Method2\_Node\_notnull-infer\_eh	      & 0    & unsat   & 0  / 0    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{}		 	& loopinv3\_Foreach.M\_System.Int32.array\_notnull-infer\_eh  & 0    & unsat   & 0  / 0    & unsat / unsat   \\
\hline                                                                                                                                               
\multicolumn{1}{|c|}{misc} 		& set14    						      & 95   & sat     & 16 / 162  & sat   / sat     \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& set16    						      & 87   & sat     & 17 / 17   & sat   / sat     \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& set19    						      & --   & TO      & TO / TO   & --    / --      \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& set1    					              & --   & TO      & TO / TO   & --    / --      \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& set2    						      & --   & TO      & TO / TO   & --    / --      \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& set3    						      & 0    & unsat   & 0  / 0    & unsat / unsat   \\
\cline{2-6}                                                                                                                                          
\multicolumn{1}{|c|}{} 			& set9    						      & 6    & sat     & 18 / 17   & sat   / sat     \\
\hline                                                                                                                                                                                            
\end{tabular}
} % End of \resizebox
\end{minipage}
\caption{Experiment results of running Z3 on the Z3/CVCx difficult ($\ge1$/$\ge10$) benchmarks of the SMT-COMP/AUFLIA-p without and with the \emph{sufGT} simplification. ``TO'': denotes time-out of 600 sec., ``UK'': denotes that the solver returns ``unknown'' before reaching time-out}
\end{table}



==> future_work.tex <==
% !TEX root =  a.a.elghazi_m.taghdiri_smt2013.draft02.tex
%---------------------
\section{Future Work}
\label{sect:future-work}



==> proofs_v2.tex <==
% !TEX root =  a.a.elghazi_m.taghdiri_smt2013.draft02.tex
\section{Proofs}
\label{a:sect:proofs}

\begin{corollary}%{col:1}
\label{col:1}
If $\vgts{x} \neq \infty$, then $\pi_x(v) \in M(\vgts{x})$, for all $v \in |M|$.
\end{corollary}

\begin{proof}
If $x$ does not occur as an argument of an uninterpreted function, then the claim follows directly from the definition of $\pi_x$. 
Otherwise, we can assume that $x$ occurs at the $i$-th argument of an uninterpreted function $f$. 
In this case, we have  $\pi_x = \pi_x(f,i)$. Because of rule $R_1$, we also have  $\n{fGT}(f,i)_\sa = \vgts{x}$, 
which, together with the definition of $\pi_x(f,i)$, implies the claim. 
\end{proof}


\begin{corollary}
\label{col:2}
For all $gt \in \n{Gr}(A)$, $M^{\pi_x}(gt) = M(gt)$.
\end{corollary}

\begin{proof}
By induction over the structure of $gt$. If $gt \in \n{Const}$, the claim follows directly from the definition of $M^{\pi_x}$. 
If, without loss of generality, $gt := f(t)$, where $f \in \n{Fun}$ and $t \in Gr$, we get by the induction hypothesis, $M^{\pi_x}(f(t)) = M^{\pi_x}(f)(M^{\pi_x}(t)) {\buildrel\rm i.h. \over=} M^{\pi_x}(f)(M(t))$. 
Now we have to distinguish between interpreted and uninterpreted functions. If $f$ is interpreted, the claim follows directly from the definition of $M^{\pi_x}$. 
If $f$ is uninterpreted, we get $M^{\pi_x}(f)(M(t)) = M(f)(\pi_x(f,1)(M(t)))$. Furthermore, we know, because of rule $R_2$ and $gt \in \n{Gr}(A)$, that $t \in \n{fGT}(f,1)_\sa$. 
Now we can use the definition of $\pi_x(f,1)$ and we get $\pi_x(f,1)(M(t)) = M(t)$.
\end{proof}


For a variable assignment $\beta$, a value $v \in |M|$ and a variable $x \in Var$, we use the notation $\beta_{x}^{v}$ to denote the modification of $\beta$ where $x$ is mapped to $v$.  

%\begin{lemma}
%\label{a:lemma:1}
%Let $M$ be a model and $\beta$ a variable assignment, then for all interpreted literals $l$ in $A$, $(M^{\pi}, \beta) \not\models l \Rightarrow (M, \beta_{y, \n{sufGT}(y)_{\scs_A} \neq \infty}^{\pi_y(\beta(y))}) \not\models l$.
%\end{lemma}
%
\begin{lemma}%{lemma:1}
\label{lemma:1}
Let $x$ be a variable with $\vgts{x} \neq \infty$, $\mc{M}$ a model, $\beta$ a variable assignment, and 
$\beta' = \lambda y.\ \n{if}\ \vgts{y} = \vgts{x} \ \n{then}\ \pi_x(\beta(y))\ \n{else}\ \beta(y)$.
Then  
$(M, \beta') \models l$ implies $(M^{\pi_x}, \beta) \models l$
for all interpreted literals $l$ in $A$.
%$(M^{\pi_x}, \beta) \not\models l \Rightarrow (M, \beta_{y, \n{vGT}(y)_{\scs_A} \neq \infty}^{\pi_y(\beta(y))}) \not\models l$.
\end{lemma}


%\begin{proof}
%%By case distinctions over the different interpreted operators. Because $\n{vGT(x)}_{\scs_A} \neq \infty$ and the rules of $\scs_A$ we can restrict w.l.o.g $l_i$ to $l_i := op(x, gt_0)$, where $op \in \{=, <, \leq, >, \geq\}$. Let now assume that $(M^{\pi_x}, \beta_{x}^{v}) \not\models l_i$ and $(M, \beta_{x}^{\pi_x(v)}) \models l_i$. For $op := \verb+"+<\verb+"+$, we get from rule $R_5$, $gt_0 \in \n{vGT(x)}_{\scs_A}$ and from the assumptions the inequality system $(v \ge gt_0) \foand (\pi_x(v) < gt_0)$, which implies that $|v - \pi_x(v)|$ is not minimal, since $|v-gt_0|$ is is more minimal. For $op \in \{\leq, >, \geq\}$ the proof is analog to the previous case. For $op := \verb+"+=\verb+"+$, we get from rule $R_{12}$, $\{gt_0-1, gt_0+1\} \subseteq \n{vGT(x)}_{\scs_A}$ and from the assumptions the inequality system $(v \not = gt_0) \foand (\pi_x(v) = gt_0)$, which is equivalent to $((v \leq gt_0-1) \foor (gt_0+1 \leq v)) \foand (\pi_x(v) = gt_0)$ and implies that $|v - gt_0|$ is not minimal, since in the case $(v \leq gt_0-1)$, $|v - (gt_0-1)|$ is more minimal and in the case $(gt_0+1 \leq v)$, $|v - (gt_0+1)|$ is more minimal.  
%%%%%%
%%%%%%
%If $\vgt{x}_{\scs_A} = \infty$ for all variables $x$ of $l$, then the claim can be shown by induction on the structure of interpreted literals. 
%Otherwise and because of the rules $R_4$ and $R_6$ we can restrict w.l.o.g $l$ to $l := op(x, gt_0)$, where $op \in \{=, <, \leq, >, \geq\}$ and $\vgt{x}_{\scs_A} \neq \infty$. 
%Lets now assume that $(M^{\pi}, \beta) \not\models l$ and $(M, \beta_{x}^{\pi_x(\beta(x))}) \models l$. 
%For $op := \verb+"+<\verb+"+$, we get from rule $R_5$, $gt_0 \in \n{vGT(x)}_{\scs_A}$ and from the assumptions the inequality system $(\beta(x) \ge gt_0) \foand (\pi_x(\beta(x)) < gt_0)$, 
%which implies that $|\beta(x) - \pi_x(\beta(x))|$ is not minimal, since $|\beta(x) - gt_0|$ is is more minimal. 
%For $op \in \{\leq, >, \geq\}$ the proof is analog to the previous case. For $op := \verb+"+=\verb+"+$, we get from rule $R_{12}$, $\{gt_0-1, gt_0+1\} \subseteq \n{vGT(x)}_{\scs_A}$ 
%and from the assumptions the inequality system $(\beta(x) \not = gt_0) \foand (\pi_x(\beta(x)) = gt_0)$, which is equivalent to $(\beta(x) \leq gt_0-1) \foor (gt_0+1 \leq \beta(x))) \foand (\pi_x(\beta(x)) = gt_0)$ 
%and implies that $|\beta(x) - gt_0|$ is not minimal, since in the case $(\beta(x) \leq gt_0-1)$, $|\beta(x) - (gt_0-1)|$ is more minimal and in the case $(gt_0+1 \leq \beta(x))$, $|\beta(x) - (gt_0+1)|$ is more minimal.  
%\end{proof}
\begin{proof}
%If $\vgts{y} = \infty$ for all variables $y$ of $l$, then $\beta' = \beta$ and $x$ do not occurs in $l$. In this case the claim can be shown by induction on the structure of interpreted literals. 
If $\vgts{y} \neq \vgts{x}$ for all variables $y$ of $l$, then $\beta' = \lambda y. \ \beta(y)$ and $x$ does not occur in $l$. 
In this case, one can easily show, by induction on the structure of expressions, that $(M^{\pi_x}, \beta)(l) = (M, \beta)(l)$. 
Otherwise and because of the rules $R_4$ and $R_6$, without loss of generality, we can restrict $l$ to $l := op(x, gt_0)$ where $op \in \{=, <, \leq, >, \geq\}$ and $\beta'$ to $\beta'= \lambda y. \ \beta_{x}^{\pi_x(\beta(x))}(y)$. 
Let us now assume that $(M, \beta_{x}^{\pi_x(\beta(x))}) \models l$ and $(M^{\pi_x}, \beta) \not\models l$. 
For $op := \verb+"+<\verb+"+$, we get from rule $R_5$, $gt_0 \in \n{vGT(x)}_{\scs_A}$ and from the assumptions the inequality system $(\beta(x) \ge gt_0) \foand (\pi_x(\beta(x)) < gt_0)$, 
which implies that $|\beta(x) - \pi_x(\beta(x))|$ is not minimal, since $|\beta(x) - gt_0|$ is strictly smaller. 
For $op \in \{\leq, >, \geq\}$, the proof is similar to the previous case. For $op := \verb+"+=\verb+"+$, we get from rule $R_{13}$, $\{gt_0-1, gt_0+1\} \subseteq \n{vGT(x)}_{\scs_A}$ 
and from the assumptions, the inequality system $(\beta(x) \not = gt_0) \foand (\pi_x(\beta(x)) = gt_0)$, which is equivalent to $(\beta(x) \leq gt_0-1) \foor (gt_0+1 \leq \beta(x))) \foand (\pi_x(\beta(x)) = gt_0)$ 
and implies that $|\beta(x) - gt_0|$ is not minimal, since in the case $(\beta(x) \leq gt_0-1)$, $|\beta(x) - (gt_0-1)|$ is strictly smaller and in the case $(gt_0+1 \leq \beta(x))$, $|\beta(x) - (gt_0+1)|$ is strictly smaller.  
\end{proof}

Lemma \ref{lemma:2} provides a stronger result compared to lemma \ref{lemma:1}. It better reflects the intuition behind the rules $R_5$, $R_7$ to $R_{13}$. 
They guarantee that if a variable $x$ occurs as an argument of an interpreted operator, then there is at least one $gt_l \in \vgts{x}$ with $\not \models_{\mathcal{T}} l[gt_l/x]$. 
That is, $C[gt_l/x]$ is either valid or its satisfiability is determined by literals other than $l$. 
We proved lemma \ref{lemma:1} because it is sufficient for our main theorem, and it has a shorter proof.

\begin{lemma}
\label{lemma:2}
Let $C$ be a clause in $A$, $x$ a variable in $C$ with $\n{vGT(x)}_{\scs_A} \neq \infty$, and $M$ a model  of $C[\n{vGT(x)}_{\scs_A}/x]$, then either there exists an uninterpreted literal $l \in C$, where $M \models l[gt/x]$ for some $gt \in \n{vGT(x)}_{\scs_A}$, or there exists a (tautology) subclause $C'$ of $C$ whose literals are interpreted and $\models_{\mathcal{T}} C'$.
\end{lemma}


In the following, we use \emph{expressions} to refer to both terms and formulas. That is, $Expr = Term \cup For$.

\begin{lemma}%{lemma:3}
\label{lemma:3}
%Let $x$ be a variable with $\vgts{x} \neq \infty$, $\mc{M}$ a model and $\beta$ a variable assignment, then for all uninterpreted literals $l$ in $A$,
%$
%(M,\beta_{y, \n{sufGT}(y)_\sa \neq \infty}^{\pi_y(\beta(y))})(l)
%= 
%(M^{\pi_x}, \beta)(l) 
%$.
Let $x$ be a variable with $\vgts{x} \neq \infty$, $\mc{M}$ a model, $\beta$ a variable assignment, and 
$\beta' = \lambda y.\ \n{if}\ \vgts{y} \neq \vgts{x} \ \n{then}\ \pi_x(\beta(y))\ \n{else}\ \beta(y)$.
Then 
$
(M,\beta')(l)
= 
(M^{\pi_x}, \beta)(l) 
$ for all uninterpreted literals $l$ in $A$.
\end{lemma}

\begin{proof}
  In order to use induction on the structure of $l$, we consider a super set of the literals, namely the expressions, excluding  variables ($Expr \setminus Var$).

  If $l$ is a ground term in $A$, then the claim follows directly from corollary \ref{col:2}. 
  
  Let $l = f(t_{1:n})$ be a function application in $A$ with $f$ an uninterpreted function. 
  The evaluations of $l$ are
  \begin{align*}
	  (M^{\pi_x},\beta)(f(t_{1:n})) &= M^{\pi_x}(f)((M^{\pi_x}, \beta)(t_1), \dots, (M^{\pi_x}, \beta)(t_n))\\
    \quad &= M(f)(\pi_x(f,1)((M^{\pi_x}, \beta)(t_1)), \dots, \pi_x(f,n)(t_n))\\
    (M, \beta')(f(t_{1:n}) &= M(f)((M,\beta')(t_1), \dots, (M,\beta')(t_n))
  \end{align*}
  It suffices to show that 
  $\pi_x(f,i)((M^{\pi_x}, \beta)(t_i)) = 
  (M, \beta')(t_i)$. 
  We do this by a case distinction over the type of the terms $t_i$.
  
  If $t_i = y$ is a variable with $\vgts{y} \neq \vgts{x}$, then $\beta'(y) = \beta(y)$ 
  and because $y$ occurs in $f$ and rule $R_1$, $\vgts{x} \neq \n{fGT}(f,i)_\sa$, which implies that
  $\pi_x(f,i)$ is the identity.

  If $t_i = y$ is a variable with $\vgts{y} = \vgts{x}$,
  then $\beta'(y) = \pi_x(\beta(y))$ and $\pi_x = \pi_x(f,i)$, because of the definition of $\pi_x$ and Rule 1.

  If $t_i$ is a function application, we assume $t_i = s[x_{1:m}]$ for some term $s$. 
  By induction hypothesis,
  $\pi_x(f,i)((M^{\pi_x}, \beta)(s[x_{1:m}])) \eqih$ 
  $\pi_x(f,i)((M, \beta')(s[x_{1:m}]))$. 
  W.r.t. $\n{fGT}(f,i)_\sa$, there is two possible cases to consider:\\
  1) $\n{fGT}(f,i)_\sa \neq \vgts{x}$, then the claim follows directly from the definition of $\pi_x(f,i)$. \\
  2) $\n{fGT}(f,i)_\sa = \vgts{x}$, this implies that, because of rule $R_3$ and $\vgts{x} \neq \infty$, 
  for all $1 \leq i \leq m$, $\vgts{x_i} \neq \infty$. 
  Using this fact together with corollary \ref{col:1}, there exists for each $x_i$ a ground term $gt_i$, 
  with $\pi_{x_i}(\beta(x_i)) = M(gt_i)$ and $gt_i \in \vgts{x_i}$.
  So we can write, $\pi_x(f,i)((M, \beta')(s[x_{1:m}])) = \pi_x(f,i)(M(s[gt_{1:m}]))$.
  Because of rule $R_3$ we know that $s[gt_{1:m}] \in \n{fGT}(f,i)_\sa$, and so $M(s[gt_{1:m}]) \in M(\n{fGT}(f,i)_\sa)$. 
  Finally the claim follows from the definition of $\pi_x(f,i)$ for values in $M(\n{fGT}(f,i)_\sa)$.

  %\achraf{[I need here (or above) to emphasis why I am excluding the case in which variables occurs as argument of an interpreted function. It has to do with the definition of $\pi_x$ for such variables \dots]}

  %Let $l := f(t_{1:n})$ be a term with $f$ an interpreted symbol. 
  %\achraf{To use induction on the $t_i$s we require that no variable occures in a $t_i$ as argument of an interpreted function. 
  %But this is guarantee by the definition of uninterpreted terms.}
  %%The $t_i$ cannot be variables, otherwise $l$ would be an interpreted term.
  %Using the definition of $M^{\pi}$ and the induction hypothesis,
  %$(M^{\pi}, \beta)(f(t_{1:n})) =$ 
  %$M^{\pi}(f)((M,\byp)(t_1), \dots, (M,\byp)(t_n))$. Using the definition of $M^{\pi}$ for interpreted functions, the claims follows directly.
  
  Let $l := f(t_{1:n})$ be an expression with $f$ an interpreted function. 
  Using the definition of $M^{\pi_x}$ for interpteded functions,
  $(M^{\pi_x}, \beta)(f(t_{1:n})) =$ 
  $M(f)((M^{\pi_x},\beta)(t_1), \dots, (M^{\pi_x},\beta)(t_n))$. 
  Since $l$ is uninterpreted, all $t_i$s are non-variables and we can use the induction hypotheses on them and get,
  $M(f)((M^{\pi_x},\beta)(t_1), \dots, (M^{\pi_x},\beta)(t_n)) =$
  $M^{\pi_x}(f)((M,\beta')(t_1), \dots, (M,\beta')(t_n))$.
  Now the claim follows directly from the definition of $M^{\pi_x}$ for interpreted functions.

\end{proof}



%\begin{proof}
%  By induction on the structure of $l$. Variables are not considered
%  in the claim, nothings needs to be shown for them.
%
%  Let $l = f(t_1, ..., t_n)$ be an uninterpreted term (possibly with
%  $n=0$) in $A$ with $f$ an uninterpreted symbol. The evaluations of
%  $l$ are
%  \begin{align*}
%    (M^\pi,\beta)(f(t_1, ..., t_n)) &= M^{\pi}(f)((M^{\pi},
%    \beta)(t_1), \cdots, (M^{\pi}, \beta)(t_n))\\
%    \quad &= M(f)(\pi(f,1)((M^{\pi}, \beta)(t_1)), ...,
%    \pi(f,n)(...))\\
%    (M, \beta_y^\pi)(f(t_1, ..., t_n) &=
%    M(f)((M,\beta_y^\pi)(t_1), ..., (M,\beta_y^\pi)(t_n))
%  \end{align*}
%  It suffices to show that $\pi(f,i)((M^{\pi}, \beta)(t_i) = (M,
%  \beta_y^\pi)(t_i)$. We do this by a case distinction over the type
%  of the terms $t_i$.
%  
%  If $t_i = x$ is a variable with $\vgts{x} = \infty$, then $\beta(x) =
%  \beta_y^\pi(x)$ and $\pi(f,i)$ is the identity (def of $pi(f,i)$ and
%  Rule 1).
%
%  If $t_i = x$ is a variable with $\vgts{x} \neq \infty$, then ...
%
%  If $t_i = g(...)$ is a function application. $g(...)$ cannot be an
%  interpreted term, because otherwise $l$ would be, too.  [the
%  induction hypothesis can be applied to $g(...)$].
%
%  \bigskip
%%\matt{[Usually struc. ind. means: 1. Let $l$ be variable and 2. Let $l=f(t_1,...,t_n)$ be application.]}
%
%If $l$ is a ground term, then the claim follows directly from corollary \ref{col:2}. 
%
%If $l := f(x_{1:n})$, lets assume w.l.o.g. that $f$ is uninterpreted and $\vgts{x_i} \neq \infty$ only for $1\leq i \leq m$, then 
%$(M^{\pi}, \beta)(f(x_{1:n})) = M^{\pi}(f)((M^{\pi}, \beta)(x_1), \cdots, (M^{\pi}, \beta)(x_n)) =$ \\ 
%$M(f)(\pi(f,1)(\beta(x_1)), \cdots, \pi(f,m)(\beta(x_m)), \pi(f,m+1)(\beta(x_{m+1})), \cdots, \pi(f,n)(\beta(x_n))) $. 
%Because each $x_i$ occurs at the $i$-th argument of $f$, we get with rule $R_1$ that $\n{vGT}(x_i) = \n{fGT}(f,i)$ especially for $1 \leq i \leq m$, which implies that $\pi_{x_i} = \pi(f,i)$ for all $1 \leq i \leq m$. 
%Now, we just need to show that $\pi(f,i)$ is the identity function for all $m < i$, but this follows from the definition of $\pi(f,i)$, rule $R_1$, and our assumption that $\n{vGT}(x_i) = \infty$ for all $m < i$.
%
%If $l := f(t(x_{1:n}))$, with $f$ uninterpreted, then  
%$(M^{\pi}, \beta)(f(t(x_{1:n}))) = 
%M^{\pi}(f)((M^{\pi},\beta)(t(x_{1:n}))) {\buildrel\rm i.h.\over=}$ \\ 
%%\matt{[$t[x_{1:n}]$ can\textbf{not} be a literal, I do not think that the i.h. can be applied. Perhaps the claim must be extended to all subterms of $A$. Only then can the i.h. be applied]}\\
%$M^{\pi}(f)((M,\beta_{y, \n{sufGT}(y) \neq \infty}^{\pi(\beta(y))})(t(x_{1:n}))) =$ $M(f)(\pi(f,1)((M,\beta_{y, \n{sufGT}(y) \neq \infty}^{\pi(\beta(y))})(t(x_{1:n}))))$. Now we need to show that, 
%$\pi(f,1)((M,\beta_{y, \n{sufGT}(y) \neq \infty}^{\pi(\beta(y))})(t(x_{1:n}))) = (M,\beta_{y, \n{sufGT}(y) \neq \infty}^{\pi(\beta(y))})(t(x_{1:n}))$. 
%W.r.t. $\n{fGT}(f,1)$, there is two possible cases to consider:\\
%1) $\n{fGT}(f,1) = \infty$, then the claim follows directly from the definition of $\pi(f,1)$. \\
%2) $\n{fGT}(f,1) \neq \infty$, this implies because of rule $R_3$ that for all $1 \leq i \leq n$, $\n{vGT}(x_i) \neq \infty$. Using this fact we get, 
%$(M,\beta_{y, \n{sufGT}(y) \neq \infty}^{\pi(\beta(y))})(t(x_{1:n})) = M(t(\pi_{x_1}(\beta(x_1)), \dots, \pi_{x_n}(\beta(x_n))))$, and $\pi_{x_i}(\beta(xi)) \in \n{vGT}(x_i)$. 
%Now because of rule $R_3$ we get $M(t(\pi_{x_1}(\beta(x_1)), \dots, \pi_{x_n}(\beta(x_n)))) \in \pi(f,1)$, and because of the definition of $\pi(f,1)$ the claim.
%
%If $l := f(t(x_{1:n}))$, with $f$ interpreted but $x$ don't occurs as argument of an interpreted operator in $l$. As in the previous case we get
%$(M^{\pi}, \beta)(f(t(x_{1:n}))) =$ 
%$M^{\pi}(f)((M,\beta_{y, \n{sufGT}(y) \neq \infty}^{\pi(\beta(y))})(t(x_{1:n})))$
%, and using the definition of $M^{\pi}$ for interpreted we get the claim.
%
%\end{proof}




==> varElimLimitAlg.tex <==
% !TEX root =  a.a.elghazi_m.taghdiri_smt2013.draft02.tex
%------------------------------------------------------------------------------
\begin{algorithm}
\KwData{$A: For, IQ_{max}: \mathbb{N}$}
\KwResult{$expVar: Set\unary{Var}$}
\Begin{
 $\n{NE} \gets \{x \in A \mid \vgts{x} = \infty\}$ \;
 \Repeat{$unchanged(\n{NE})$}{
  \For{$x \in A \setminus \n{NE}$}{
   $sc_x \gets scope(x)$ \;
   \While{$sc_x \neq \emptyset$}{
    $cost_x \gets (\prod\limits_{y \in s_x\setminus \n{NE}} \vgts{y}) * |s_x \cap \n{NE}|$ \; 
    \If{$cost_x > IQ_{max}$}{
     $sc_x \gets sc_x \setminus y \in \{y \in sc_x \mid |\vgts{y}| = \max\limits_{z \in sc_x}(\vgts{z})\}$ \;
     $\n{NE} \gets \n{NE} \setminus \{y\}$ 
    }
   }
  }
 }
 \Return{$expVar$}
}
\caption{Heuristic detection of expensive variables, w.r.t. $IQ_{max}$}
\label{algo:qbi2}
\end{algorithm}

